Reprogrammable, in-materia matrix-vector multiplication with floppy modes

Matrix-vector multiplications are a fundamental building block of artificial intelligence; this essential role has motivated their implementation in a variety of physical substrates, from memristor crossbar arrays to photonic integrated circuits. Yet their realization in soft-matter intelligent systems remains elusive. Here, we experimentally demonstrate a reprogrammable elastic metamaterial that computes matrix-vector multiplications using floppy modes -- deformations with near-zero stored elastic energy. Floppy modes allow us to program complex deformations without being hindered by the natural stiffness of the material; but their practical application is challenging, as their existence depends on global topological properties of the system. To overcome this challenge, we introduce a continuously parameterized unit cell design with well-defined compatibility characteristics. This unit cell is then combined to form arbitrary matrix-vector multiplications that can even be reprogrammed after fabrication. Our results demonstrate that floppy modes can act as key enablers for embodied intelligence, smart MEMS devices and in-sensor edge computing.

==> matvec.tex <==
\begin{tikzpicture}
    \node[] (in0) at (0,0) {$x_0$};
    \node[] (in1) at (0,-3) {$x_1$};
    \node[] at (0,-6) {$\vdots$};
    \node[] at (1.5,-6) {$\vdots$};
    \node[] at (3.5,-6) {$\vdots$};
    \node[] at (5.5,-6) {$\vdots$};
    \node[] at (7.5,-6) {$\vdots$};

    \node[] (inn) at (0,-7) {$x_n$};
    \node[] (out0) at (2,-10) {$X_0$};
    \node[] (out1) at (4,-10) {$X_1$};
    \node[] at (5.5,-10) {$\ldots$};
    \node[] at (5.5,-8) {$\ldots$};
    \node[] at (5.5,-4) {$\ldots$};
    \node[] at (5.5,-1) {$\ldots$};

    \node[] (outN) at (8,-10) {$X_N$};

    \draw[-stealth] (in0.east) -- ++ (8,0);
    \draw[-stealth] (in1.east) -- ++ (8,0);
    \draw[-stealth] (inn.east) -- ++ (8,0);

    \node[draw=black, 
        circle,
        minimum size=0.3cm,
        inner sep=0
        ] (prod00) at (1,-1){$\Large \times$};

    \node[draw=black, 
        circle,
        minimum size=0.3cm,
        inner sep=0
        ] (prod10) at (1,-4){$\Large \times$};

    \node[draw=black, 
        circle,
        minimum size=0.3cm,
        inner sep=0
        ] (prod20) at (1,-8){$\Large \times$};


    \node[draw=black, 
        circle,
        minimum size=0.3cm,inner sep=0,
        ] (sum00) at (2,-1){$\Large + $};

    \node[draw=black, 
        circle,
        minimum size=0.3cm,inner sep=0,
        ] (prod01) at (3,-1){$\Large \times$};

    \node[draw=black, 
        circle,
        minimum size=0.3cm,inner sep=0,
        ] (prod11) at (3,-4){$\Large \times$};

    \node[draw=black, 
        circle,
        minimum size=0.3cm,inner sep=0,
        ] (prod21) at (3,-8){$\Large \times$};
        
    \node[draw=black, 
        circle,
        minimum size=0.3cm,inner sep=0,
        ] (sum01) at (4,-1){$\Large + $};

    \node[draw=black, 
        circle,
        minimum size=0.3cm,inner sep=0,
        ] (prod03) at (7,-1){$\Large \times $};
        
    \node[draw=black, 
        circle,
        minimum size=0.3cm,inner sep=0,
        ] (prod13) at (7,-4){$\Large \times $};
        
    \node[draw=black, 
        circle,
        minimum size=0.3cm,inner sep=0,
        ] (prod23) at (7,-8){$\Large \times $};
        
    \node[draw=black, 
        circle,
        minimum size=0.3cm,inner sep=0,
        ] (sum03) at (8,-1){$\Large + $};

    \node[draw=black, 
        circle,
        minimum size=0.3cm,inner sep=0,
        ] (sum10) at (2,-4){$\Large + $};

    \node[draw=black, 
        circle,
        minimum size=0.3cm,inner sep=0,
        ] (sum11) at (4,-4){$\Large + $};
        
    \node[draw=black, 
        circle,
        minimum size=0.3cm,inner sep=0,
        ] (sum13) at (8,-4){$\Large + $};

    \node[draw=black, 
        circle,
        minimum size=0.3cm,inner sep=0,
        ] (sum20) at (2,-8){$\Large + $};

    \node[draw=black, 
        circle,
        minimum size=0.3cm,inner sep=0,
        ] (sum21) at (4,-8){$\Large + $};
        
    \node[draw=black, 
        circle,
        minimum size=0.3cm,inner sep=0,
        ] (sum23) at (8,-8){$\Large + $};

    \draw[-stealth] (prod00.east) -- (sum00.west);
    \draw[-stealth] (prod01.east) -- (sum01.west);
    \draw[-stealth] (prod03.east) -- (sum03.west);

    \draw[-stealth] (prod10.east) -- (sum10.west);
    \draw[-stealth] (prod11.east) -- (sum11.west);
    \draw[-stealth] (prod13.east) -- (sum13.west);

    \draw[-stealth] (prod20.east) -- (sum20.west);
    \draw[-stealth] (prod21.east) -- (sum21.west);
    \draw[-stealth] (prod23.east) -- (sum23.west);

    \draw[-stealth] (1,0) -- (prod00.north) ;
    \draw[-stealth] (3,0) -- (prod01.north) ;
    \draw[-stealth] (7,0) -- (prod03.north) ;

    \draw[-stealth] (1,-3) -- (prod10.north);
    \draw[-stealth] (3,-3) -- (prod11.north);
    \draw[-stealth] (7,-3) -- (prod13.north);

    \draw[-stealth] (1,-7) -- (prod20.north);
    \draw[-stealth] (3,-7) -- (prod21.north);
    \draw[-stealth] (7,-7) -- (prod23.north);

    \node[draw=black, 
        rectangle,
        ] (alpha00) at (1,-2){$\large \alpha _ {00}$};

    \node[draw=black, 
        rectangle,
        ] (alpha01) at (1,-5){$\large \alpha _ {01}$};
    
    \node[draw=black, 
        rectangle,
        ] (alpha02) at (1,-9){$\large \alpha _ {0n}$};

    \node[draw=black, 
        rectangle,
        ] (alpha10) at (3,-2){$\large \alpha _ {10}$};

    \node[draw=black, 
        rectangle,
        ] (alpha11) at (3,-5){$\large \alpha _ {11}$};
    
    \node[draw=black, 
        rectangle,
        ] (alpha12) at (3,-9){$\large \alpha _ {1n}$};

    \node[draw=black, 
        rectangle,
        ] (alpha20) at (7,-2){$\large \alpha _ {N0}$};

    \node[draw=black, 
        rectangle,
        ] (alpha21) at (7,-5){$\large \alpha _ {N1}$};
    
    \node[draw=black, 
        rectangle,
        ] (alpha22) at (7,-9){$\large \alpha _ {Nn}$};


    \draw[-stealth] (alpha00.north) -- (prod00.south);
    \draw[-stealth] (alpha10.north) -- (prod01.south);
    \draw[-stealth] (alpha20.north) -- (prod03.south);

    \draw[-stealth] (alpha01.north) -- (prod10.south);
    \draw[-stealth] (alpha11.north) -- (prod11.south);
    \draw[-stealth] (alpha21.north) -- (prod13.south);

    \draw[-stealth] (alpha02.north) -- (prod20.south);
    \draw[-stealth] (alpha12.north) -- (prod21.south);
    \draw[-stealth] (alpha22.north) -- (prod23.south);
    
    \draw[-stealth] (sum00.south) -- (2,-2.75);
    \draw[-stealth] (sum01.south) -- (4,-2.75);
    \draw[-stealth] (sum03.south) -- (8,-2.75);

    \draw[-stealth] (sum10.south) -- (2,-5.5);
    \draw[-stealth] (sum11.south) -- (4,-5.5);
    \draw[-stealth] (sum13.south) -- (8,-5.5);

    \draw[-stealth] (sum20.south) -- (out0.north);
    \draw[-stealth] (sum21.south) -- (out1.north);
    \draw[-stealth] (sum23.south) -- (outN.north);

    \draw[-stealth] (2,-2.75)  to [bend left=45]  (sum10.north);
    \draw[-stealth] (4,-2.75)  to [bend left=45]  (sum11.north);
    \draw[-stealth] (8,-2.75)  to [bend left=45]  (sum13.north);


    \draw[-stealth] (2,-6.75)  to [bend left=45]  (sum20.north);
    \draw[-stealth] (4,-6.75)  to [bend left=45]  (sum21.north);
    \draw[-stealth] (8,-6.75)  to [bend left=45]  (sum23.north);
        \end{tikzpicture}

